Dynamical metasurfaces: electromagnetic properties and instabilities

In this thesis, I analyse the electromagnetic properties of dynamical metasurfaces and find two critical phenomena. The first is the Casimir-induced instability of a deformable metallic film. In general, two charge-neutral interfaces attract with or repel each other due to the contribution from the zero-point fluctuation of the electromagnetic field between them, namely, the Casimir effect. The effects of perturbative interface corrugation on the Casimir energy in the film system is studied by the proximity force approximation with dispersion correction. If the corrugation period exceeds a critical value, the Casimir effect dominates the surface tension and brings about structural instability. The second is \v{C}erenkov radiation in the vacuum from a time-varying, corrugated surface. Travelling faster than light brings about electromagnetic shock waves, \v{C}erenkov radiation. Since light is the fastest object in a vacuum, it has been considered that \v{C}erenkov radiation is emitted only in the presence of some refractive index. Here, I propose mimicking a series of particles travelling faster than light in a vacuum by dynamical surface corrugation to find \v{C}erenkov radiation in a vacuum from the surface. The dynamical corrugation induces an effective current source on the surface with an external electrostatic field applied. When the corrugation profile is of travelling wave type, the source can be regarded as a series of dipoles virtually travelling along the surface. If the phase velocity of the travelling wave profile exceeds the speed of light, and so do the dipoles, they emit \v{C}erenkov radiation in a vacuum.

==> introduction/contributions.tex <==
\section{Contributions}

Contributions here.

